Verifiable and Compositional Reinforcement Learning Systems

We propose a framework for verifiable and compositional reinforcement learning (RL) in which a collection of RL subsystems, each of which learns to accomplish a separate subtask, are composed to achieve an overall task. The framework consists of a high-level model, represented as a parametric Markov decision process (pMDP) which is used to plan and to analyze compositions of subsystems, and of the collection of low-level subsystems themselves. By defining interfaces between the subsystems, the framework enables automatic decompositions of task specifications, e.g., reach a target set of states with a probability of at least 0.95, into individual subtask specifications, i.e. achieve the subsystem's exit conditions with at least some minimum probability, given that its entry conditions are met. This in turn allows for the independent training and testing of the subsystems; if they each learn a policy satisfying the appropriate subtask specification, then their composition is guaranteed to satisfy the overall task specification. Conversely, if the subtask specifications cannot all be satisfied by the learned policies, we present a method, formulated as the problem of finding an optimal set of parameters in the pMDP, to automatically update the subtask specifications to account for the observed shortcomings. The result is an iterative procedure for defining subtask specifications, and for training the subsystems to meet them. As an additional benefit, this procedure allows for particularly challenging or important components of an overall task to be determined automatically, and focused on, during training. Experimental results demonstrate the presented framework's novel capabilities.

==> algorithms/icrl.tex <==


\begin{algorithm}[t]
    \DontPrintSemicolon 
    \KwIn{ Partially instantiated sub-systems \(\controllerSet = \{\controller_1, \controller_2, ..., \controller_{\numControllers}\}\), \(\hlmFailProb\), \(\trainingSteps\), \(\maxTrainingSteps\).}
    \KwOut{Sub-system policies \(\{\policy_{\controller_1}, \policy_{\controller_2}, ..., \policy_{\controller_{\numControllers}}\}\), meta-policy \(\abstractPolicy\).}
    
    \(\abstractMDP \gets ConstructHLM(\controllerSet)\)\;
    
    \(\{\policy_{\controller_1}, \policy_{\controller_2}, ..., \policy_{\controller_{\numControllers}}\} \gets instantiateSubSystemPolicies()\)\; 
    
    \(\abstractPolicy \gets instantiateMetaPolicy()\)\;

    \(\controllerPerformanceEstimate_{\controller_1}, \controllerPerformanceEstimate_{\controller_2}, ..., \controllerPerformanceEstimate_{\controller_{\numControllers}}, \controllerPerformanceEstimate_{\abstractPolicy} \gets 0\); \(\numSteps_{\controller_1}, \numSteps_{\controller_2}, ..., \numSteps_{\controller_{\numControllers}} \gets 0\)\;
    
    \(\lbList \gets \{\controllerPerformanceEstimate_{\controller_1}, \controllerPerformanceEstimate_{\controller_2}, ..., \controllerPerformanceEstimate_{\controller_{\numControllers}}\}\); \(\ubList \gets \{\}\)\;
    
    % \For{$i \in \{1,2,...,\numControllers\}$}{
    %     \(\policy_{\controller_i} \gets RLTrain(\controller_i, \policy_{\controller_i}, \initTrainingSteps)\)\;
    %     \(\controllerPerformanceEstimate_{\controller_i}(\cdot) \gets estimateSubTaskSuccessProbability(\controller_i, \policy_{\controller_i})\)\;
    %     \(\abstractMDP \gets updateHLM(\abstractMDP, \controllerPerformanceEstimate_{\controller_i})\)\;
    %     % \For{\(\mdpState \in \controllerInitialStateSet_{\controller_i}\)}{
    %     %     \(\controllerPerformanceEstimate_{\controller_i}(\mdpState) \gets estimateSubTaskSuccessProbability(\controller_i, \mdpState)\)\;
    %     % }
    % }
    
    \While{\(\controllerPerformanceEstimate_{\abstractPolicy} \leq 1 - \delta\)}{
        
        \(\{\bernoulliProb_{\controller_1}, \ldots, \bernoulliProb_{\controller_{\numControllers}}\} \gets\)
        \text{Solution of bilinear program~\eqref{eq:hlm_opt_objective}-\eqref{eq:hlm_opt_ub_constraints} using} \((\abstractMDP, \lbList, \ubList)\)\; %(\perfAwareOptProblem(\abstractMDP, \lbList, \ubList)
        
        \(\controller_{j} \gets selectSubSystemToTrain(\bernoulliProb_{\controller_1}, \bernoulliProb_{\controller_2}, ..., \bernoulliProb_{\controller_{\numControllers}}, \controllerPerformanceEstimate_{\controller_1}, \controllerPerformanceEstimate_{\controller_2},..., \controllerPerformanceEstimate_{\controller_{\numControllers}})\)\;
    
        \(\policy_{\controller_{j}} \gets RLTrain(\controller_j, \policy_{\controller_j}, \trainingSteps)\); \(\numSteps_{\controller_j} \gets \numSteps_{\controller_j} + \trainingSteps\)\;
        
        \(\controllerPerformanceEstimate_{\controller_j} \gets estimateSubTaskSuccessProbability(\controller_j, \policy_{\controller_j})\)\;
        
        \(\lbList.update(\controllerPerformanceEstimate_{\controller_j})\)\;
        
        % \(\abstractMDP \gets updateHLM(\abstractMDP, \controllerPerformanceEstimate_{\controller_j})\)\;
        
        \If{\(\numSteps_{\controller_j} \geq \maxTrainingSteps\)}{\(\ubList.add(\controllerPerformanceEstimate_{\controller_j})\)\;}
        
        \(\abstractPolicy \gets solveOptimalHLMPolicy(\abstractMDP, \lbList)\); \(\controllerPerformanceEstimate_{\abstractPolicy} \gets predictTaskSuccessProbability(\abstractMDP, \abstractPolicy, \lbList)\)\;
    }
    
    \Return{\(\{\policy_{\controller_1}, \policy_{\controller_2}, ..., \policy_{\controller_{\numControllers}}\}\), \(\abstractPolicy\)}\;
    
    \caption{Iterative Compositional RL}
    \label{alg:ICRL}
\end{algorithm}

==> tex/09_dummy_opt_problem.tex <==
\begin{align}
    \min_{\occupancyVar, \bernoulliProb_{\controller}} \quad & \sum_{\controller \in \controllerSet} \bernoulliProb_{\controller} \\
    \textrm{s.t.} \quad &  \text{pMDP-Constraints}(\occupancyVar, \bernoulliProb_{\controller}) \\
    & \text{Task specification}(\occupancyVar, \bernoulliProb_{\controller})
\end{align}%
